Scalable Trajectory-User Linking with Dual-Stream Representation Networks

Trajectory-user linking (TUL) aims to match anonymous trajectories to the most likely users who generated them, offering benefits for a wide range of real-world spatio-temporal applications. However, existing TUL methods are limited by high model complexity and poor learning of the effective representations of trajectories, rendering them ineffective in handling large-scale user trajectory data. In this work, we propose a novel $\underline{Scal}$abl$\underline{e}$ Trajectory-User Linking with dual-stream representation networks for large-scale $\underline{TUL}$ problem, named ScaleTUL. Specifically, ScaleTUL generates two views using temporal and spatial augmentations to exploit supervised contrastive learning framework to effectively capture the irregularities of trajectories. In each view, a dual-stream trajectory encoder, consisting of a long-term encoder and a short-term encoder, is designed to learn unified trajectory representations that fuse different temporal-spatial dependencies. Then, a TUL layer is used to associate the trajectories with the corresponding users in the representation space using a two-stage training model. Experimental results on check-in mobility datasets from three real-world cities and the nationwide U.S. demonstrate the superiority of ScaleTUL over state-of-the-art baselines for large-scale TUL tasks.

==> table/Notations.tex <==
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{2mm}{}
\fontsize{9}{12}
\begin{tabular}{c|c}
\hline
\textbf{Notation} & \textbf{Definition} \\ \hline
$u$ &  a user\\
$p$ & a uniquely identified venue\\
$c$ & the category of the venue\\
$t$ & the timestamp of the check-in\\
$(u, p, c, t)$& check-in records\\
$Tr_{\tau}$   & the trajectory with a specific time interval $\tau$\\
$\mathcal{T}$   & the set of trajectories \\ 
$\mathcal{U}$ & the set of users \\
${M}_{r}$ & a binary mask vector\\
$r$ & the ratio of masking points\\
$x_{i}$ & the semantic location representation\\
$\mathbf{X}$ & the representations of all
 locations\\
 $\mathcal{F}_{\theta_{\alpha}}$ & the short-term encoder \\
  $\mathcal{F}_{\theta_{\beta}}$ & the long-term encoder \\
   $\mathcal{F}_{\theta^{\blacktriangle}_{\alpha}}$ & the frozen short-term encoder \\
  $\mathcal{F}_{\theta^{\blacktriangle}_{\beta}}$ & the frozen long-term encoder \\
$z_{\alpha}$ &  the representations of the short trajectory\\
$z_{\beta}$ &  the representations of the long trajectory\\
$\gamma$& a learnable weight \\
$z$& the final representation of dual-stream encoder\\
$z_{*}$& the representation in the unit hypersphere\\
$u_{i}$ & the user label who generated trajectory $i$\\
$y_i$ & unlinked trajectory $i$ representation\\
\hline
\end{tabular}
\caption{Notation and Definitions}
% \vspace{-3mm}
\label{tab:notations}
\end{table}

==> table/algorithm.tex <==
\begin{algorithm}
    \caption{The Learning Process of \model}
    % \fontsize{9}{12}
\setlength{\tabcolsep}{2mm}{}
    \fontsize{9}{12}\selectfont
    \label{tab-algorithm}
    \renewcommand{\algorithmicrequire}{ \textbf{Input:}}
    \renewcommand{\algorithmicensure}{ \textbf{Output:}}
   
    \begin{algorithmic}[1]
        \REQUIRE ~~\\
            Raw trajectory: $Tr_d$ \\
        \ENSURE ~~\\
            User representations u
        
        \STATE \textbf{// Stage 1: Pretraining with Contrastive Learning}
            \STATE Get $Tr^{T_{Aug}} =\{{Tr_{d}\cup {Tr_{7d}}\cup{Tr_{14d}}}\}$ from temporal augmentation;
            \STATE Get $Tr^{S_{Aug}} =Tr^{T_{Aug}} \odot {M}_{r}$ from spatial augmentation;
            \STATE $\mathbf{X}=\text{EmbeddingLayer}(Tr)$;
            \STATE  $z_{\alpha}= \mathcal{F}(\theta_{\alpha};~\mathbf{X})$ , $z_{\beta}= \mathcal{F}(\theta_{\beta};~\mathbf{X})$;  
            \STATE $z=\|(\gamma \cdot {z_{\alpha}}+(1-\gamma) \cdot {z_{\beta}})\|_2$;
            \STATE $z_*=\|Proj(z)\|_2$;
            \STATE compute contrastive loss $\mathcal{L}_{cl}$;
        % \STATE Update model parameters using gradient descent 
        
        \STATE \textbf{// Stage 2: Fine-tuning with Trajectory-User Linking}
        % \FOR{each trajectory $Tr_{\tau}$ in $\mathcal{T}$}
        \STATE ${z}=\|(\gamma \cdot {\mathcal{F}(\theta^{\blacktriangle}_{\alpha};~\mathbf{X})}+(1-\gamma) \cdot {\mathcal{F}(\theta^{\blacktriangle}_{\beta};~\mathbf{X})})\|_2$;
        \STATE ${u}_{i}=\operatorname{Average-Pooling}(\{z^j|j\in U_i\})$;
        \STATE $y=f(\theta;~z)$;
        \STATE Minimize cosine similarity loss $\mathcal{L}_{ul}$ between $y_i$ and corresponding user representation $u_{i}$;

        
        \RETURN u;
    \end{algorithmic}
\end{algorithm}





==> table/parameter.tex <==
\begin{table}[h!]
\centering
\fontsize{9}{12}
\setlength{\tabcolsep}{2mm}{}
\begin{tabular}{c|cc}
\hline
\textbf{Hyperparameters} & $f_{\theta_{\alpha}}$ & $f_{\theta_{\beta}}$ \\ \hline
POI embedding dimension         & 512 & 512 \\ 
Category embedding dimension         & 512 & 512 \\ 
Time embedding dimension        & 128 & 128 \\ 
Check-in embedding dimension    & 512 & 512 \\ 
Hidden size                     & 1024 &  \textbackslash \\ 
Layers                          & 1 & 1 \\ 
Model dimension&               \textbackslash & 512\\
State dimension          & \textbackslash & 128 \\ 
Conv dimension            & \textbackslash & 2 \\ 
Expand             & \textbackslash & 2 \\ 
\midrule
Training epochs                 & \multicolumn{2}{c}{100} \\ 
Batch size                      & \multicolumn{2}{c}{512} \\ 
Adam $\epsilon$                 & \multicolumn{2}{c}{1e-8} \\ 
Adam $\beta$                    & \multicolumn{2}{c}{(0.9, 0.999)} \\
Initial learning rate in 1st stage           & \multicolumn{2}{c}{1e-3} \\ 
Initial learning rate in 2nd stage           & \multicolumn{2}{c}{5e-4} \\ 
Learning rate schedule in 1st stage        & \multicolumn{2}{c}{multi (5,0.9)} \\ 
Learning rate schedule in 2nd stage        & \multicolumn{2}{c}{multi (5,0.1)} \\ 
Dropout                         & \multicolumn{2}{c}{0.1} \\ 
Mask ratio                         & \multicolumn{2}{c}{0.9} \\ 
\hline
\end{tabular}
\caption{Hyperparameters for model.}
\label{tab:parameters}
\end{table}
